Learning Plannable Representations with Causal InfoGAN

In recent years, deep generative models have been shown to 'imagine' convincing high-dimensional observations such as images, audio, and even video, learning directly from raw data. In this work, we ask how to imagine goal-directed visual plans -- a plausible sequence of observations that transition a dynamical system from its current configuration to a desired goal state, which can later be used as a reference trajectory for control. We focus on systems with high-dimensional observations, such as images, and propose an approach that naturally combines representation learning and planning. Our framework learns a generative model of sequential observations, where the generative process is induced by a transition in a low-dimensional planning model, and an additional noise. By maximizing the mutual information between the generated observations and the transition in the planning model, we obtain a low-dimensional representation that best explains the causal nature of the data. We structure the planning model to be compatible with efficient planning algorithms, and we propose several such models based on either discrete or continuous states. Finally, to generate a visual plan, we project the current and goal observations onto their respective states in the planning model, plan a trajectory, and then use the generative model to transform the trajectory to a sequence of observations. We demonstrate our method on imagining plausible visual plans of rope manipulation.

==> improvement.tex <==
\section{Loss Improvement}
\TODO{Depending on how much self-consistency loss helps, we might move it to ablation study in experiment section.}
To further strengthen the relationship between transitions in the abstract model and the real observations, we propose to add a self-consistency loss on the transitions, by maximizing the likelihood of observed transitions in the classified states. Namely, let $s^*(o) = \argmax_s Q(s|o)$ denote the most likely state encoding for an observation, then the self-consistency loss is given by, 
%% TK: In theory, we don't need argmax and can use the distribution given by Q(s|o) to compute self-consistency loss.
%% AT: That's true, but for sake of clarity, not sure we want to delve into it here. Do you think it is important to add?
\begin{equation*}
    L_{\text{SC}}(\theta) = \mathbb{E}_{o,o'\sim \PD} \left[ -\log T_{\model}(s^*(o') | s^*(o))\right].
\end{equation*}
Finally, we have the complete Causal InfoGAN loss function:
\begin{equation}\label{eq:CI_loss_full}
    \min_{G,Q,\model} \max_D \quad V(G, D) - \lambda_{\text{VLB}} I_{\text{VLB}}(G,Q) - \lambda_{\text{SC}} L_{\text{SC}}(\theta),
\end{equation}
where $\lambda_{\text{VLB}}$ and $\lambda_{\text{SC}}$ are parameters that control the weight of the different loss terms.
